Level-strategyproof Belief Aggregation Mechanisms

In the problem of aggregating experts' probabilistic predictions over an ordered set of outcomes, we introduce the axiom of level-strategy\-proofness (level-SP) and prove that it is a natural notion with several applications. Moreover, it is a robust concept as it implies incentive compatibility in a rich domain of single-peakedness over the space of cumulative distribution functions (CDFs). This contrasts with the literature which assumes single-peaked preferences over the space of probability distributions. Our main results are: (1) a reduction of our problem to the aggregation of CDFs; (2) the axiomatic characterization of level-SP probability aggregation functions with and without the addition of other axioms; (3) impossibility results which provide bounds for our characterization; (4) the axiomatic characterization of two new and practical level-SP methods: the proportional-cumulative method and the middlemost-cumulative method; and (5) the application of proportional-cumulative to extend approval voting, majority rule, and majority judgment methods to situations where voters/experts are uncertain about how to grade the candidates/alternatives to be ranked.\footnote{We are grateful to Thomas Boyer-Kassem, Roger Cooke, Aris Filos-Ratsikas, Herv\'e Moulin, Clemens Puppe and some anonymous EC2021 referees for their helpful comments and suggestions.} \keywords{Probability Aggregation Functions \and ordered Set of Alternatives \and Level Strategy-Proofness \and Proportional-Cumulative \and Middlemost-Cumulative}

==> drop.tex <==
\begin{itemize}
    \item \textit{IIA}:  This is because MJ is transitive and the ranking between two candidates $A$ and $B$ by MJU depends only on their distributions $p^{A}$ and $p^{B}$, which are only a function of the inputs regarding them.
    \item \textit{Impartiality}: candidates are treated equally by the method. This is because MJ is impartial and MJU applies the same PAF (the weighted-proportional-cumulative) to compute each candidate's $A$ distribution $p^A$. If we want the method to be \textit{anonymous} (voters are treated equally) just set $w_1=\dots=w_N=\frac{1}{N}$.
    \item \textit{Extends MJ}: if all voters are certain about their choices (i.e. their input are Dirac measures) and have equal weights (anonymity), MJU outputs the empirical distribution of inputs for each candidate, and so the ranking of MJU coincides with the ranking of MJ. Note that proportional-cumulative is the only level-SP method that induces an extension of MJ. 
    \item \textit{Resistance to strategic manipulations}: This is because the proportional-cumulative is level-SP and MJ was designed to counter strategic manipulations.
\end{itemize}


In this section we explore what it means to have weighted experts and characterize all the Level-SP methods in that case. 

To express our axioms, the pool of participating experts will vary, and a set of experts can be removed from the pool and others can replace him.  We assume that we have an infinite (non countable) set of potential experts $W$. Each expert has a fixed non-negative weight $(w_i)_{i\in W}$. We only consider situations where a finite subset of experts $M \subset W$ are asked to participate. 

A WPAF $\psi_{\textbf{W}}$ associates to each finite subset $M$ of $W$ a PAF $\psi_{\textbf{W}}^M:\mathcal{P}^M\rightarrow \mathcal{P}$. When $\psi_{\textbf{W}}^M$ is Level-SP for every $M$, $\psi_{\textbf{W}}$ is called Level-SP and, we denote by $f_S^M(a)$ the associated phantom function. 

For a finite $M \subset W$ and $i\in M$, we let  $M_{-i}$ denote $M$ without $i$ ($M_{-i} = M - \{i\}$). 


The next axiom means that if we replace an expert by several experts that have the same input as him and such that the sum of their weights is worth his, the outcome of the PAF is unchanged. We assume $W$ is rich enough for such replacements to always be possible.

\begin{axiom}[Weight additivity.]
A WPAF $\psi_\textbf{W}$ is weight additive if:

\begin{align*}
    \forall M \text{finite} \subseteq W, \forall S \ \text{finite} \  \subset W -M, \forall i\in M, \forall \textbf{p} \in \mathcal{P}^{M \cup S}, \\
    (w_i = \sum_{j \in S} w_j) \wedge (\forall j \in S, p_i = p_j) \Rightarrow \psi_{\textbf{W}}^{M_{-i} \cup S}(\textbf{p}_{M_{-i}},\textbf{p}_S) = \psi_{\textbf{W}}^M(\textbf{p}_M).
\end{align*}
\end{axiom}



The next axiom says that if all experts have their weights multiplied by a same positive value the outcome of the PAF remains the same (again, $W$ is assumed rich enough for replacements to always be feasible).

\begin{axiom}[Weights proportionality.]
A WPAF is weight proportional if for all $M \subset W$ and $K \subset W$, if there is $\kappa>0$ and a bijection $h : M \rightarrow K$ such that for all $i\in M, w_{h(i)}=\kappa w_i$ then 

\[\forall \textbf{p} \in \mathcal{P}^{M\cup K},
(\forall i \in M, p_{i} = p_{h(i)}) \Rightarrow
\psi_{\textbf{W}}^M(\textbf{p}_M) = \psi_{\textbf{W}}^K(\textbf{p}_K). \]
\end{axiom}


\begin{theorem}
       A Level-strategyproof WPAF $\psi_{\textbf{W}}$ is weight proportional and additive iff there exists a function $\gamma: \Lambda \times [0,1] \rightarrow [0,1]$ right continuous and none-decreasing in its first argument, and none-decreasing in its second argument with for all $a$, $\lim_{a \rightarrow \sup \Lambda}g(a,1)=1$; such that once the none-empty subset of participating experts $M\subset W$ is defined, the associated phantom functions $f_S^M$ all verify:

    \[f_S^M(a) =\gamma\left(a,\frac{\sum_{j \in S} w_j}{\sum_{j\in M}w_j} \right).\]

    And in that case, the cumulative of $\psi_{\textbf{W}}^M$ can be computed as follows:

    \[\forall a\in\Lambda, \forall \textbf{P} \in \mathcal{C}^M, \Psi_{\textbf{W}}^M(\textbf{P})(a) := \sup \left\{ y | \dfrac{\sum_{i: P_i(a) \geq y}w_i}{\sum_{i \in N}w_i} \geq \gamma(a,y) \right\}.\] 
\end{theorem}

\proof{Proof}
$\Rightarrow:$ For this proof we will use the notation $w(S) := \sum_{j\in S}w_i$.
\begin{itemize}
    \item First let us show that $\gamma$ exists. Suppose there exists $S,M,S',M'$ such that $\dfrac{w(S)}{w(M)} = \dfrac{w(S')}{w(M')}$. Let us consider the situation where all experts $i \in S \cup S'$ have $P_i(a) =1$ and all other experts in $M \cup M'$ have $P_i(a) =0$.
Then according to "weight additivity", we can replace by a two sets of two experts $M_2 =\{1,2\}$ and $M'_2 =\{1',2'\}$ such that experts $1,2,1',2'$ have respectfully weights $w(S),w(M)-w(S),w(S'),w(M')-w(S)$. We also have $P_1(a) = P_{1'}(a) = 1$ and $P_2(a) = P_{2'}(a) = 0$. By "weight proportionality", we can multiply the weights of $M'_2$ to obtain the weights of $M_2$. Therefore our two settings have identical outcomes. It follows that  $f_S^M(a) = f_{S'}^{M'}(a)$. 

We have shown that when $\dfrac{w(S)}{w(M)} = \dfrac{w(S')}{w(M')}$ we have $f_S^M(a) = f_{S'}^{M'}(a)$. We can therefore find a function $\gamma$ such that for all $S$ and $M$ $f_S^M(a) = \gamma\left(a,\frac{w(S)}{w(M)} \right)$.
\item Let us now show that $\gamma$ is none-decreasing in its second argument. Suppose this is false. Then there are $S,M,S',M'$ and $a\in \Lambda$ such that $\dfrac{w(S)}{w(M)} < \dfrac{w(S')}{w(M')}$ and $\gamma\left(a,\dfrac{w(S)}{w(M)}\right) > \gamma\left(a,\dfrac{w(S')}{w(M')}\right)$. Let us consider the situation where all experts $i \in S \cup S'$ have $P_i(a) =1$ and all other experts in $M \cup M'$ have $P_i(a) =0$. 

By "weight proportionality", by multiplying all the weights in the $M'$ setting by a constant, we can obtain $w(M)=w(M')$ (Note this could mean that in the two settings a same player has two different weights, this is not an issue since the settings are treated independently). It follows that we have $w(S) < w(S')$. By "weight additivity", we can now consider the settings as having three experts $M_3=\{1,2,3\}$. The expert $1$ has weight $w(S)$ and $P_1(a)=1$. The expert $2$ has weight $w(M)+w(M')-w(S)-w(S')$ and $P_2(a)=0$ and finally expert $3$ has weight $w(S')$, in the first setting we have $P_3(a)=1$ and in the second setting $P_3(a)=0$. It follows that $ f_S^{M_3}(a) > f_{S \cup S'}^{M_3}(a)$ which is absurd (because a phantom function much be monotone).
\item The remaining conditions are necessary to ensure that the phantom functions are none-decreasing right-continuous and that $\lim_{a \rightarrow \sup \Lambda} f_M^M(a) = 1$ 
\end{itemize}
$\Leftarrow:$ Suppose that $\gamma$ exists. It is immediate that the PAF "weight additive" and "weight proportional".\Halmos
\endproof







